A Scoping Study of Evaluation Practices for Responsible AI Tools: Steps Towards Effectiveness Evaluations

Responsible design of AI systems is a shared goal across HCI and AI communities. Responsible AI (RAI) tools have been developed to support practitioners to identify, assess, and mitigate ethical issues during AI development. These tools take many forms (e.g., design playbooks, software toolkits, documentation protocols). However, research suggests that use of RAI tools is shaped by organizational contexts, raising questions about how effective such tools are in practice. To better understand how RAI tools are -- and might be -- evaluated, we conducted a qualitative analysis of 37 publications that discuss evaluations of RAI tools. We find that most evaluations focus on usability, while questions of tools' effectiveness in changing AI development are sidelined. While usability evaluations are an important approach to evaluate RAI tools, we draw on evaluation approaches from other fields to highlight developer- and community-level steps to support evaluations of RAI tools' effectiveness in shaping AI development practices and outcomes.

==> effectivenessframework.tex <==
\begin{table}[t]
\centering
\caption{An example effectiveness evaluation framework}
\label{tab:framework}
%\resizebox{\textwidth}{!}{%
%\fontsize{3.5}{4}\selectfont
\begin{tabular}{@{}cp{6cm}p{8cm}@{}}
\toprule
\begin{tabular}[t]{@{}l@{}}\st{Reflection}\\ \st{point}\end{tabular} & \st{Description} & \st{Worked example for a tool for documenting training dataset characteristics} \\ \midrule
\st{1)} 
& \st{\textbf{Identify the goals of the RAI tool} as concretely as possible (e.g., in terms of changes to development processes or system outcomes).} 
& \st{The goal of the dataset documentation tool is to ensure downstream users of the dataset know how to use it for tasks or contexts for which the dataset is appropriate.}\\

\st{2)} 
& \st{\textbf{Determine relevant stakeholders} whose input should inform evaluation design to achieve that goal, particularly when defining `effectiveness' and selecting an evaluation method.}
& \st{Data workers (the intended users of the tool); practitioners who will use the documentation to inform decision-making; and representatives of communities who may be included in the dataset (e.g., artists whose art is in the LAION dataset }\cite{Shan2023-tc}\st{) or who are impacted by the system the data is used to train.}\\

\st{3)} 
& \st{\textbf{Articulate a theory of change} for how the tool might achieve these intended goals, within a specific context (e.g., in terms of a sequence of causal relationships beginning with use of the RAI tool during AI development).} 
& \st{\textit{If} documentation creators use the tool to record relevant characteristics of datasets, and \textit{if} practitioners review a dataset's documentation before deciding to use it, \textit{then} training datasets will only be used in training tasks for which they are appropriate.}\\

\st{4)}
& \st{\textbf{Define `effectiveness' of the tool }in the contexts identified, in terms of relevant indicators or measures to assess impact of the tool on intermediate behaviors, activities, or processes that constitute the theory of change, as well as impact on measures of intended goals.}\looseness=-1 
& \st{A measure of documentation creators' ability to identify the relevant characteristics of datasets to include in documentation }\cite[eg.,][]{Gu2021-bl}\st{; likelihood of documentation consumers reviewing, and taking action based on, a dataset's documentation before use; reduction in number of incidents of dataset misuse.}\\

\st{5)} 
& \st{\textbf{Select evaluation method} that enables data to be collected on the relationship between use of RAI tool and the indicators, measures, or metrics identified as proxies for `effectiveness'.}
& \st{A think-aloud study of documentation creators to assess their ability to use the protocol; workshop with product teams, using completed dataset documentation to review and select a dataset for a given training task; a longitudinal study in which product teams record dataset decisions on a weekly basis.}\\

\st{6)} 
& \st{\textbf{Reflect on and document findings} from the evaluation method that are likely to generalize to contexts, use cases, and intended users outside of the evaluation setting and sample.}
& \st{Think-aloud in-lab settings may not account for time pressures on documentation creators, which impact use of the protocol; study conducted within a single workplace, which may not be representative of other workplaces; during workshops and longitudinal study, participants may be performative.}\\ \bottomrule
\end{tabular}%
%}
\end{table}
